Listening to Chaotic Whispers: A Deep Learning Framework for News-oriented Stock Trend Prediction

Stock trend prediction plays a critical role in seeking maximized profit from stock investment. However, precise trend prediction is very difficult since the highly volatile and non-stationary nature of stock market. Exploding information on Internet together with advancing development of natural language processing and text mining techniques have enable investors to unveil market trends and volatility from online content. Unfortunately, the quality, trustworthiness and comprehensiveness of online content related to stock market varies drastically, and a large portion consists of the low-quality news, comments, or even rumors. To address this challenge, we imitate the learning process of human beings facing such chaotic online news, driven by three principles: sequential content dependency, diverse influence, and effective and efficient learning. In this paper, to capture the first two principles, we designed a Hybrid Attention Networks to predict the stock trend based on the sequence of recent related news. Moreover, we apply the self-paced learning mechanism to imitate the third principle. Extensive experiments on real-world stock market data demonstrate the effectiveness of our approach.

==> section/discussion.tex <==
Although the proposed framework has achieved promising results, there still exist some limitations in our work that lack to be solve in the future.

First, there exist some bias in our simulation experiments. As is shown in the Figure\ref{fig:cumulative}, the overall market trend in the testing set is rising, indicating that although our framework can get a promising result in a bullish market, it is uncertain whether it can still work in a relatively bearish market. This requires us to conduct more extensive experiments to test the performance as well as enlarging the dataset scale.

Second, the preprocessing methods used in our experiments only retain the articles that contains at least one stock name. Although such methods can filter out the unrelated news, it undoubtedly will let out model skip many informative news. To solve this limitation, we have to employ some more fine-grained preprocessing techniques to model the relationship between any news piece and the stock.

Third, our method only process the news as plain text by embedding each document using an unsupervised Word2Vec. However, such processing technique neither cannot explicitly model more fine-grained information in the news, such as the event and the relationship of event with the stocks, not can it incorporate any outside domain-knowledge knowledge, such as the properties and business domain of each stocks. To solve this limitation, we have to encode each document in a more fine-grained approach, and extract some higher-dimensional features from the news. For example, the work conducted by Ding extract the event in each news explicitly and encode each event using a knowledge-graph based embedding. This processing method can be a potential enhancement of our framework.

Forth, our method only uses the news information as the prediction clue, rather than incorporating the technical factors mined from price and volume sequence. As a matter of fact, these factors are not only informative to the stock trend prediction, but also beneficial for better comprehending the news content. Thus, it's meaningful to incorporate the some technical factors into our framework to see if it can enhance the performance.





==> section/problem.tex <==
In this section, we briefly describe how we collect the stock and news dataset used in our experiments and their formats. Then, we present the definition of the stock trend prediction classification task as our problem setting, while specifying the feature input and label output.

% \subsection{Chinese stock Data}

We obtained the Chinese stock data, including price and trading volume from 2014 to 2017 in daily frequency. There are totally 2527 stocks, covering the vast majority of Chinese stocks.

% \subsection{On-line News Data}

% \begin{figure}[ht]
% \centering   
% \includegraphics [width=0.5\textwidth]{./picture/newsamount.png} 
% \caption{News amount varied by time, each data point is the news amount within one week.} 
%  \label{fig:amount} 
% \end{figure}

\begin{figure}[ht]
\centering   
\includegraphics [width=0.45\textwidth]{./picture/dist.png} 
\caption{Probability distribution of the rise percent.} 
 \label{fig:dist} 
\end{figure}

We collected $1,271,442$ economic news between 2014 and 2017\footnote{The news data are collected from two famous economic websites in China, which are ~\url{http://www.eastmoney.com/} and ~\url{http://finance.sina.com.cn/}. We plan to release the dataset in the future.}. For each news, we extracted the publication time-stamp, title, and its content. 

For each stock $s$, we only collect the news sentences that contains the stock name and regarded them as the news sentences related to $s$. 
%Such simple mapping method may undoubtedly skip a lot of informative news which does not contain any stock names but are highly related to them, but it can filter irrelevant news to avoid noise, which is significant for our later analysis. We can use some finer-grained preprocessing methods in the future work.
%
After such processing, the total news amount is $425,250$. We then aggregate all the news in date $t$ to construct the news corpus for this day, denoted as $C_t= [n_{t1}, n_{t2}, ..., n_{tL}]$, where %$C_t$ denotes the news corpus at time-stamp $t$, and 
$n_{ti}$ denotes the $i^{th}$ news in this corpus $C_t$.

% \subsection{problem definition}

We regard the problem of stock trend prediction as a classification problem. For a given date $t$ and a given stock $s$, 
%we can calculate the rise percent of the stock price compared to the next date $t+1$ by:
we can calculate the rise percent for the subsequent date $t+1$ by:

$Rise\_Percent(t+1) = \frac{Close\_Price(t+1) - Close\_Price(t)} {Close\_Price(t)}$

Based on the rise percent, the date $t$ can be binned into three $Next\_Rise\_Label(t)$: \textit{DOWN} ($Rise\_Percent(t+1) < -1\%$), \textit{UP} ($Rise\_Percent(t+1) > 1\%$), \textit{PRESERVE} ($|Rise\_Percent(t+1)| \leq 1\%$). We define the thresholds so that the three categories are approximately even, as is shown in Figure~\ref{fig:dist}. 

Although there exist some other prediction targets, such as the regression task that predicts the rise percent directly, or the binary classification task that only use Rise or Down as labels. The reason of choosing the tri-label classification is the trade off between the model capacity and the learning difficulty. 

One the one hand, for real-world trading, a classification model can only predict the probability of each stock to go rise, while a precise regression model can directly estimate the rise percent, based on which the profits can be maximized. However, such a precise regression model is too hard to learn based on the chaotic market data, while classification task simplifies the stock trend, reducing the learning difficulty. 

On the other hand, the ultimate pursue of investors is profit. In the setting of binary classification, the samples with a very low positive rise percent will be labeled as positive. Even if the model can accurately assign such samples, the investors can hardly gain promising profits by them. On the contrary, since the tri-label classification task explicitly distinguish a class of samples with small market trend fluctuation, denoted as \textit{PRESERVE} label, the \textit{UP} samples it successfully classified can gain a profit ratio of at least $1\%$, which is quite a large profit for each day.

Therefore, our task can be formulated as the following: given a time sequence length $N$, the stock $s$ and date $t$, use the news corpus sequence from time $t-N+1$ to $t$, denoted as $[C_{t-N+1}, C_{t-N+2}, ..., C_{t-1}, C_t]$, to make the prediction of $Next\_Rise\_Label(t)$, indicating the price trend of stock $s$ for the subsequent date $t+1$. Each news corpus $C_i$ contains a set of news with the size of $L$, $C_i = [n_{i1}, n_{i2}, ..., n_{iL}]$. 
%The task is to design a model to classify the $Rise\_Label(t)$, indicating the market trend of the next time stamp $t$. 
Intuitively, 
%most of the event influence to 
the influence of news on 
a price trend is similar among different stocks. Therefore, we simply build one single classifier to accomplish this task.
